SLACK: Attacking LiDAR-based SLAM with Adversarial Point Injections

The widespread adoption of learning-based methods for the LiDAR makes autonomous vehicles vulnerable to adversarial attacks through adversarial \textit{point injections (PiJ)}. It poses serious security challenges for navigation and map generation. Despite its critical nature, no major work exists that studies learning-based attacks on LiDAR-based SLAM. Our work proposes SLACK, an end-to-end deep generative adversarial model to attack LiDAR scans with several point injections without deteriorating LiDAR quality. To facilitate SLACK, we design a novel yet simple autoencoder that augments contrastive learning with segmentation-based attention for precise reconstructions. SLACK demonstrates superior performance on the task of \textit{point injections (PiJ)} compared to the best baselines on KITTI and CARLA-64 dataset while maintaining accurate scan quality. We qualitatively and quantitatively demonstrate PiJ attacks using a fraction of LiDAR points. It severely degrades navigation and map quality without deteriorating the LiDAR scan quality.

==> images/WACV-ADV <==
<mxfile host="app.diagrams.net" modified="2023-08-30T13:29:22.301Z" agent="Mozilla/5.0 (Windows NT 10.0; Win64; x64) AppleWebKit/537.36 (KHTML, like Gecko) Chrome/115.0.0.0 Safari/537.36 Edg/115.0.1901.203" etag="v4oks3piy9XGwTLnm1Qx" version="21.7.1" type="device" pages="2">
  <diagram name="Page-1" id="ekC30iSoMj9A6b82Shjx">
    <mxGraphModel dx="815" dy="524" grid="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" page="1" pageScale="1" pageWidth="827" pageHeight="1169" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-1" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=-0.003;entryY=0.195;entryDx=0;entryDy=0;entryPerimeter=0;startArrow=none;startFill=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-3" target="XMF6G12HVGVJ6vwZhX7I-4" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-2" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=0;exitY=0.5;exitDx=0;exitDy=0;entryX=0.75;entryY=0;entryDx=0;entryDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-3" target="XMF6G12HVGVJ6vwZhX7I-25" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-3" value="" style="triangle;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="160" y="230" width="50" height="60" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-4" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#e1d5e7;strokeColor=#9673a6;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="320" y="230" width="126.91" height="150" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-5" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=0;exitY=0.5;exitDx=0;exitDy=0;entryX=1;entryY=0.5;entryDx=0;entryDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-6" target="XMF6G12HVGVJ6vwZhX7I-4" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-6" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$1$$&lt;/font&gt;" style="text;html=1;strokeColor=#b85450;fillColor=#f8cecc;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="510" y="280" width="60" height="50" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-7" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=-0.005;entryY=0.796;entryDx=0;entryDy=0;entryPerimeter=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-9" target="XMF6G12HVGVJ6vwZhX7I-4" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-8" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=0;exitY=0.5;exitDx=0;exitDy=0;entryX=0.75;entryY=1;entryDx=0;entryDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-9" target="XMF6G12HVGVJ6vwZhX7I-26" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-9" value="" style="triangle;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="160" y="320" width="50" height="60" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-10" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=0;exitY=0.25;exitDx=0;exitDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-12" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="280" y="260" as="targetPoint" />
            <Array as="points">
              <mxPoint x="280" y="148" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-11" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=0;entryY=0.5;entryDx=0;entryDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-12" target="XMF6G12HVGVJ6vwZhX7I-15" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-12" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#e1d5e7;strokeColor=#9673a6;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="680" y="90" width="126.91" height="150" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-13" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=-0.003;entryY=0.797;entryDx=0;entryDy=0;entryPerimeter=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-14" target="XMF6G12HVGVJ6vwZhX7I-12" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-14" value="" style="triangle;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="550" y="180" width="50" height="60" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-15" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$1$$&lt;/font&gt;" style="text;html=1;strokeColor=#b85450;fillColor=#f8cecc;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="870" y="140" width="60" height="50" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-16" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=1;exitY=0.5;exitDx=0;exitDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-17" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="650" y="210" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-17" value="" style="triangle;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;rotation=-180;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="756.91" y="340" width="50" height="60" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-18" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=0;exitY=0.75;exitDx=0;exitDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-20" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="240" y="350" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-19" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=0;exitY=0.25;exitDx=0;exitDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="XMF6G12HVGVJ6vwZhX7I-20" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="630" y="210" as="targetPoint" />
            <mxPoint x="806.91" y="475" as="sourcePoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-20" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#a9b3c1;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="830" y="430" width="100" height="60" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-21" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\textbf{MMD}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="850" y="445" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-22" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\textbf{PD}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="353" y="290" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-23" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\textbf{Recon}(k,\bar k)$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="850" y="355" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-24" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$d_j$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="90" y="230" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-25" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$d_{jseg}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="90" y="260" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-26" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$s_j$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="90" y="320" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-27" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$s_{jseg}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="90" y="350" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-28" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;$$\textbf{KITTI}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="480" y="210" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-29" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;$$\textbf{KITTI}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="480" y="170" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-30" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;$$\textbf{MASK}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="480" y="234" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-31" value="" style="group" parent="1" vertex="1" connectable="0">
          <mxGeometry x="310" y="20" width="410" height="40" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-32" value="" style="rounded=0;whiteSpace=wrap;html=1;" parent="XMF6G12HVGVJ6vwZhX7I-31" vertex="1">
          <mxGeometry width="410" height="40" as="geometry" />
        </mxCell>
        <mxCell id="XMF6G12HVGVJ6vwZhX7I-33" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\textrm{Unsupervised Domain Adaptation (UDA)}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="XMF6G12HVGVJ6vwZhX7I-31" vertex="1">
          <mxGeometry x="175" y="5" width="60" height="30" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
  <diagram id="4fwntwesItKVld4eKjP6" name="Page-2">
    <mxGraphModel dx="815" dy="524" grid="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" page="1" pageScale="1" pageWidth="827" pageHeight="1169" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-1" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=1;exitY=0.5;exitDx=0;exitDy=0;entryX=-0.003;entryY=0.195;entryDx=0;entryDy=0;entryPerimeter=0;startArrow=none;startFill=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="9qkOUaf6tpqxD0FsZO6D-3" target="9qkOUaf6tpqxD0FsZO6D-4" edge="1">
          <mxGeometry relative="1" as="geometry">
            <Array as="points">
              <mxPoint x="330" y="559" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-3" value="&lt;font style=&quot;font-size: 21px;&quot;&gt;$$AE_{seg}$$&lt;/font&gt;" style="triangle;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="220" y="508" width="110" height="100" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-4" value="" style="rounded=0;whiteSpace=wrap;html=1;fillColor=#e1d5e7;strokeColor=#9673a6;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="400" y="530" width="126.91" height="150" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-5" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=0;exitY=0.5;exitDx=0;exitDy=0;entryX=1;entryY=0.5;entryDx=0;entryDy=0;endArrow=none;endFill=0;strokeWidth=2;" parent="1" source="9qkOUaf6tpqxD0FsZO6D-6" target="9qkOUaf6tpqxD0FsZO6D-4" edge="1">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-6" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$1$$&lt;/font&gt;" style="text;html=1;strokeColor=#b85450;fillColor=#f8cecc;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="590" y="580" width="60" height="50" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-10" value="&lt;font style=&quot;font-size: 18px;&quot;&gt;$$\textbf{PD}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="433" y="590" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-11" value="&lt;font style=&quot;font-size: 25px;&quot;&gt;$$s_j$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="84" y="527" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-12" value="&lt;font style=&quot;font-size: 25px;&quot;&gt;$$s_{jseg}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="87" y="557" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-13" value="&lt;font style=&quot;font-size: 25px;&quot;&gt;$$d_j$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="84" y="630" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-14" value="&lt;font style=&quot;font-size: 25px;&quot;&gt;$$d_{jseg}$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="87" y="663" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-15" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;exitX=1;exitY=0.5;exitDx=0;exitDy=0;strokeWidth=2;endArrow=none;endFill=0;" parent="1" source="9qkOUaf6tpqxD0FsZO6D-16" edge="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="340" y="560" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-16" value="" style="triangle;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;rotation=-180;strokeWidth=2;" parent="1" vertex="1">
          <mxGeometry x="432.99999999999994" y="420" width="50" height="60" as="geometry" />
        </mxCell>
        <mxCell id="9qkOUaf6tpqxD0FsZO6D-17" value="&lt;font style=&quot;font-size: 25px;&quot;&gt;$$\textbf{Recon}(s_j,d_j)$$&lt;/font&gt;" style="text;html=1;strokeColor=none;fillColor=none;align=center;verticalAlign=middle;whiteSpace=wrap;rounded=0;" parent="1" vertex="1">
          <mxGeometry x="539.9999999999999" y="435" width="60" height="30" as="geometry" />
        </mxCell>
        <mxCell id="d3Zidip3UJ9yU5WU80ou-4" value="&lt;font style=&quot;font-size: 21px;&quot;&gt;$$AE_{seg}$$&lt;/font&gt;" style="triangle;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;strokeWidth=2;" vertex="1" parent="1">
          <mxGeometry x="220" y="613" width="110" height="100" as="geometry" />
        </mxCell>
        <mxCell id="d3Zidip3UJ9yU5WU80ou-5" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;endArrow=none;endFill=0;strokeWidth=2;" edge="1" parent="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="401" y="663" as="sourcePoint" />
            <mxPoint x="325" y="663" as="targetPoint" />
            <Array as="points">
              <mxPoint x="396" y="663" />
              <mxPoint x="396" y="663" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="d3Zidip3UJ9yU5WU80ou-10" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;endArrow=none;endFill=0;strokeWidth=2;" edge="1" parent="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="219" y="665" as="sourcePoint" />
            <mxPoint x="143" y="665" as="targetPoint" />
            <Array as="points">
              <mxPoint x="214" y="665" />
              <mxPoint x="214" y="665" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="d3Zidip3UJ9yU5WU80ou-11" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;endArrow=none;endFill=0;strokeWidth=2;" edge="1" parent="1">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="220" y="563" as="sourcePoint" />
            <mxPoint x="144" y="563" as="targetPoint" />
            <Array as="points">
              <mxPoint x="215" y="563" />
              <mxPoint x="215" y="563" />
            </Array>
          </mxGeometry>
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>

